IDProtector: An Adversarial Noise Encoder to Protect Against ID-Preserving Image Generation

Recently, zero-shot methods like InstantID have revolutionized identity-preserving generation. Unlike multi-image finetuning approaches such as DreamBooth, these zero-shot methods leverage powerful facial encoders to extract identity information from a single portrait photo, enabling efficient identity-preserving generation through a single inference pass. However, this convenience introduces new threats to the facial identity protection. This paper aims to safeguard portrait photos from unauthorized encoder-based customization. We introduce IDProtector, an adversarial noise encoder that applies imperceptible adversarial noise to portrait photos in a single forward pass. Our approach offers universal protection for portraits against multiple state-of-the-art encoder-based methods, including InstantID, IP-Adapter, and PhotoMaker, while ensuring robustness to common image transformations such as JPEG compression, resizing, and affine transformations. Experiments across diverse portrait datasets and generative models reveal that IDProtector generalizes effectively to unseen data and even closed-source proprietary models.

==> backup/3-method-wr_v0.tex <==
\section{The Proposed Method}
\label{sec:method}
\begin{figure*}[!h]
    \centering
\includegraphics[width=1.\linewidth]{images/method_v4.png}
    \caption{Overall schematics of our method. }
    \vspace{-0.4cm}
    \label{method}
\end{figure*}

SSR-Encoder is built on text-to-image diffusion models~\cite{ldm}, reviewd in Sec. \ref{sec:3.1-preliminary}. It consists of two key parts: token-to-patch aligner and detail-preserving image encoder in SSR-Encoder (Sec. \ref{sec:3.2}) and subject conditioned generation process (Sec. \ref{sec:3.3}). Finally, we present the details of training strategies and loss function in Sec. \ref{sec:3.4}.

% In this section, we present the details of our method. Firstly, we introduce the overall framework of the generation pipeline(\ref{sec:3.1}). Next, we present the details of three crucial components of our approach, including the SSR-encoder(\ref{sec:3.2}), the subject-conditioned generation process(\ref{sec:3.3}), and the training strategies(\ref{sec:3.4}). 

\subsection{Preliminary for Diffusion Models}
\label{sec:3.1-preliminary}
Diffusion Model ~\cite{ddpm, scoremodel} belongs to the category of generative models that denoise from a Gaussian prior $\mathbf{x_T}$ to target data distribution $\mathbf{x_0}$ by means of an iterative denoising procedure. The common loss used in DM is:

\begin{equation}
    L_{simple}(\bm{\theta}) := \mathbb{E}_{\mathbf{x_0}, t, \bm{\eta}}\left[\left\|\bm{\eta}-\bm{\eta_\theta}\left(\mathbf{x_t}, t\right)\right\|_2^2\right] 
 \end{equation}
 where $\mathbf{x_t}$ is an noisy image constructed by adding noise $\bm{\eta} \in \mathcal{N}(\mathbf{0},\mathbf{1})$  to the natural image $\mathbf{x_0}$ and the network $\bm{\eta_\theta(\cdot)}$ is trained to predict the added noise. At inference time, data samples can be generated from Gaussian noise $\bm{\eta} \in \mathcal{N}(\mathbf{0},\mathbf{1})$ using the predicted noise $\bm{\eta_\theta}(\mathbf{x_t}, t)$ at each timestep $t$ with samplers like DDPM~\cite{ddpm} or DDIM~\cite{ddim}.

Latent Diffusion Model (LDM)~\cite{ldm} is proposed to model image representations in autoencoder’s latent space. LDM significantly speeds up the sampling process and facilitates text-to-image generation by incorporating additional text conditions. The LDM loss is:
\begin{equation}
    L_{LDM}(\bm{\theta}) := \mathbb{E}_{\mathbf{x_0}, t, \bm{\eta}}\left[\left\|\bm{\eta}-\bm{\eta_\theta}\left(\mathbf{x_t}, t, \bm{\tau_{\theta}}(\mathbf{c})\right)\right\|_2^2\right] 
 \end{equation}
 where $\mathbf{x_0}$ represents image latents and $\bm{\tau_\theta(\cdot)}$ refers to the BERT text encoder~\cite{bert} used to encodes text description $\mathbf{c}$.

Stable Diffusion (SD) is a widely adopted text-to-image diffusion model based on LDM. Compared to LDM, SD is trained on a large LAION ~\cite{laion5b} dataset and replaces BERT with the pre-trained CLIP~\cite{clip} text encoder.

\subsection{Selective Subject Representation Encoder}
\label{sec:3.2}
%Our method is based on a pre-trained diffusion model, with the overall structure as shown in Fig.\ref{method}. Firstly, given a reference image $x$ and a query input $P$ (text or mask), our SSR-Encoder outputs the subject embedding $E_{S}$, which contains the specified subject information related to query input from the reference image. Then, $E_{S}$ serves as the guide conditions for the diffusion model in different layers, guiding the image generation process together with the original text branch in the text-to-image diffusion model. 
%The overall structure of our is illustrated in Fig.\ref{method}. It begins with the input of a reference image $x$ and a query subject input $S$ (which can be text or a mask). The SSR-Encoder processes these inputs to generate the subject embedding $E_{S}$. This embedding encapsulates the targeted subject information extracted from the reference image in relation to the query input. Subsequently, $E_{S}$ is employed as a guiding condition within various layers of a pretrained stable diffusion model. It works in tandem with the original text branch of the text-to-image diffusion model to direct the generation process.
Selective subject-driven image generation aims to generate target subjects in a reference image with high fidelity and creative editability, guided by user's selective queries (text or mask). Our SSR-Encoder is specifically designed to address this problem and can be applied to any customized diffusion models without the need for test-time fine-tuning. 

Formally, given a reference image $\mathbf{x}$ and a user's query input $\mathbf{S}$, our SSR-encoder captures specific subject information and outputs multi-scale subject embeddings $\mathbf{E_{S}}$. Then, the multi-scale subject embeddings $\mathbf{E_{S}}$ are integrated into U-Net model with trainable copies of vanilla cross-attention layers. Finally, conditioned on both subject embeddings $\mathbf{E_{S}}$ and editing text embedding $\mathbf{E^e_{T}}$, we generate desired subjects with high fidelity and creative editability via subject conditioned generation process.
The overall schematics is demonstrated in Fig. \ref{method}. 

Our Selective Subject Representation Encoder (SSR-Encoder) is composed of two integral parts: Token-to-Patch Aligner and Detail-Preserving Subject Embedding. The details are as follows.



% The process initiates with the introduction of a reference image $x$ and a query subject input $S$, which can be in the form of text or a mask. At the heart of our system is the SSR-Encoder, which processes these inputs to produce the subject embedding $E_{S}$. This embedding is key; it captures the specific subject information derived from the reference image in accordance with the query input. The resulting $E_{S}$ then plays a crucial role, serving as a guiding condition across various layers of a pre-trained stable diffusion model. With the original text branch of the text-to-image diffusion model, $E_{S}$ effectively steers the image generation process.




% Moreover, based on the Multiple Cross-Attention Strategy, it works with multiple image inputs as well. This allows for the combination of different concepts from multiple reference images.

% \subsection{The SSR-Encoder}
% \label{sec:3.2}
% Our Selective Subject Representation Encoder (SSR-Encoder) is composed of two integral parts: the \textbf{Detail-Preserving Image Encoder} and the \textbf{Text-to-Image Selective Aligner}. %The \textbf{Detail-Preserving Image Encoder} in our work is based on CLIP image encoder but with multi-scale extension. It's designed to contain two crucial attributes: 1) the image encoder should extract fine details as much as possible, and 2) the extracted image feature should be well-aligned with text embedding. The \textbf{Text-to-Image Selective Aligner} serves as a bridge of text and image and extracting subject embedding $E_S$ w.r.t. the text query $T$ and reference image $I$.

%It is worth mentioning that, although only trained on the image-text pair dataset, after the text query is successfully aligned with related image patches, SSR-Encoder can naturally accept the input of mask query based on the attention mechanism.

%\textbf{Detail-Preserving Image Encoder}. The majority work of finetuning-free subject-driven generation takes usage of the global embedding or spatial embeddings from the last layer of CLIP image encoder. Though it's well-aligned with the pretrained CLIP text encoder $E_t$, the image embedding has already lost fine details. In order to ensure the preservation of image details, we take the pretrained CLIP image encoder as the base model and extract features from different layers of the encoder. Formally, the CLIP image encoder takes image $x$ as input, and output $E_I=CLIP(x)$, where $E_I={z_k\in \mathbb{R}^{257 \times 768}, k={0,...,5}}$ is the multi-scale image embedding extracted from 6 layers of the CLIP ViT image encoder.  

%As the previous finetuning-free works suffer from lack of details in the generated images, we conducted several experiments\footnote{experiment details can be found in supplimentary Sec.A} to reveal that the image embedding coming from CLIP image encoder has already discarded fine details. In contrast, our detail-preserving image encoder is capable of reconstructing fine details. Therefore, the least requirement of the image encoder is fulfilled: it does not lose information.


% This component is an adaptation of the CLIP image encoder, augmented with multi-scale capabilities. Its design focuses on two primary objectives: (1) extracting as much fine detail as possible from images, and (2) ensuring that the extracted image features align with text embeddings. Unlike conventional finetuning-free subject-driven generation approaches that predominantly rely on global or spatial embeddings from the final layer of the CLIP image encoder, our method extracts features across different encoder layers. Formally, the CLIP image encoder processes an image $x$ to produce $E_I=CLIP(x)$, where $E_I$ is a multi-scale image embedding ${z_k \in \mathbb{R}^{257 \times 768}, k={0,...,5}}$ extracted from six layers of the CLIP ViT image encoder. Our experiments\footnote{Detailed in the supplementary Section A.} demonstrate that while standard embeddings from the CLIP image encoder tend to lose fine details, our Detail-Preserving Image Encoder effectively retains and reconstructs these details, satisfying the essential requirement of information preservation in image encoding.

\textbf{Token-to-Patch Aligner}. %The purpose of the T2I aligner is to align image patch features with text token features, such that the model is capable of extracting subject embedding from reference image. Given a text-image pair with text embedding $E_T\in \mathbb{R}^{77 \times 768}$ and image embedding $E_I$, a cross attention block is employed to align them. The image embeddings $z_0$ from the last layer and text embedding $T$ are projected into the same space via respective weights $W_K$ and $W_Q$, then the attention matrix $A^{it}$ is calculated, as shown in Equ.\ref{equal1}:
As observed in many previous work ~\cite{maskclip, clipsurgery, dinoregister}, CLIP tends to prioritize background regions over foreground regions even identifying a target category. Therefore, relying solely on the similarity between texts and images may prove inadequate in capturing specific subject information. To alleviate it, we propose Token-to-Patch (T2P) Aligner, which learns two trainable linear projection to align image patch features with given text token features. Mathematically, given a query text-image pair $(\mathbf{E_T^q}, \mathbf{E^s_I})$, where the text embedding is $\mathbf{E_T^q}\in \mathbb{R}^{N_t \times D_t}$ and the semantic image embedding is $\mathbf{E^s_I}\in \mathbb{R}^{N_i \times D_i}$, we adopt projection layer $\mathbf{W^Q}$ and $\mathbf{W^K}$ to embed them into a common space. The alignment is illustrated as follows:
%image embadding z and the text embedding t is projected to the same 
%better focusing on semantically relevant areas of the image and obtaining the Selected Image Embeddings $E_{S}$ used to guide generation. Moreover, we use a layered training strategy to inject different information for different layers of stable diffusion. Specifically, we leverage the 
\begin{equation}
\label{equal:aligner}
\mathbf{Q}=\mathbf{W^Q}\cdot \mathbf{E_T^q}, \mathbf{K}=\mathbf{W^K}\cdot \mathbf{E^s_I} \\
\end{equation}

\begin{equation}
\label{equal:attn_operation}
\mathbf{A_{t2p}}=\operatorname{Softmax}\left(\frac{\mathbf{Q} \mathbf{K^{\top}}}{\sqrt{d}}\right)
\end{equation}
where $\mathbf{A_{t2p}} \in \mathbb{R}^{N_t \times N_i}$ represents the text-to-image attention map and $\mathbf{W^Q}$ and $\mathbf{W^K}$ are projection matrices for the transformation of text query and image key features. 


The $\mathbf{A_{t2p}}$ matrix serves a dual role: it identifies similarities and acts as a region selector, so our aligner naturally support \textbf{mask-based query}. In practice, we can manually assign a mask $\mathbf{M}$ to $\mathbf{A_{it}}$ for mask-guided generation with null-text query inputs. Following Equ.~\ref{equal:attn_operation}, we can reweight $\mathbf{A_{it}}$ with predefined mask $\mathbf{M}$ to emphasize selective regions. This approach ensures our SSR-encoder only focus on the selected valid regions of reference images.


\textbf{Detail-Preserving Subject Embedding}. 
Following most of previous methods~\cite{ye2023ip, pada, elite}, we use a pre-trained CLIP image encoder to extract image representation from reference image. However, the commonly used features from CLIP fall short of meeting our requirements: extracting as much fine detail as possible from images. Our preliminary experiments \footnote{Detailed in the supplementary Section A.} verify a significant degradation of fine-grained details in the vanilla image features. Hence, we propose detail-preserving subject embedding, which extracts features across different encoder layers to preserve more fine-grained details. Formally, the image encoder processes an image $\mathbf{x}$ to produce multi-scale detailed image features $\mathbf{E_I} = \{\mathbf{z_k}\}_{k=0}^{K}$, where $\mathbf{z_0}=\mathbf{E_I^s} \in \mathbb{R}^{N_i \times D_i}$ represents semantic image embedding and $\mathbf{z_k}$ represents detailed image embedding at the scale of $k$, $N_i$ represents the number of image tokens, $D_i$ represents the feature dimension of each token feature and $K$ refers to the number of target scales. 
 
To capture more fine-grained details, we adopt separate linear projection $\mathbf{W_k^V}$ for image feature $\mathbf{z_k}$ at different scales. Then, combine the text-to-image attention map $\mathbf{A_{t2p}}$, we can calculate $\mathbf{E_S}=\{\mathbf{E^k_S}\}^K_{k=0}$ following Equ.\ref{subject_projection}:
\begin{equation}
\label{subject_projection}
\mathbf{V_k}=\mathbf{W^V_k}\cdot \mathbf{z_k}, \\
\mathbf{E^k_{S}}={\mathbf{A_{t2p}} \mathbf{V^{\top}_k}},
\end{equation}
where $\mathbf{E^k_S}$ denotes selective subject representation at scale of $k$, and $\mathbf{W^V_k}$ denotes the projection matrix for the transformation of image feature $\mathbf{z_k}$. 

Our SSR-encoder now enable to capture multi-scale subject representation $\mathbf{E_S}=\{\mathbf{E_S^k}\}_{k=0}^K$, which are then used for selective subject-driven image generation via subject conditioned generation process.
%As shown in Fig\ref{image8}, after training on a large amount of paired image-text datasets, our cross-attention module has acquired the ability to match the corresponding region of text and image. This capability is key to achieving selective subject-driven generation.

%\vspace{-0.3cm}
%\subsubsection{Query Modalities}
%\textbf{Text query input.} Text query input is a user-friendly flexible and fast approach, requiring only the user to be able to describe their thoughts without relying on other additional operations which has always been difficult to achieve in the past. For text query input, the SSR-Encoder uses the CLIP text encoder to extract text features as query input. With the help of our Layered Cross-Attention Modules, we can efficiently use the text features to query corresponding image patches. 

%\textbf{Mask query input.} The $A_{t2p}$ not only identifies similarity, but it also performs as a region selector. In the application, we can also manually assign a mask to $A_{t2p}$. Mask-guided generation is a side job of the SSR encoder. Specifically, we use the text features of the empty text and image features of the input image to input the SSR-Encoder and calculate cross-attention. Then, with a predefined mask, we can reweight $A_{t2p}$ such that the valid regions are emphasized while the impact of the invalid region is correspondingly reduced. In this way, we can make the Subject Embeddings output by SSR-Encoder only contain information about the image of the valid region we selected. 
% \textbf{Mask Query Input}. The $A_{t2p}$ matrix serves a dual role: it identifies similarities and acts as a region selector. In practice, we can manually assign a mask to $A_{it}$ for mask-guided generation, a complementary function of the SSR encoder. This involves using the text features of an empty text and the image features of the input image as inputs to the SSR-Encoder and calculating cross-attention. By applying a predefined mask, we can reweight $A_{it}$ to emphasize valid regions while diminishing the impact of invalid regions. This approach ensures that the Subject Embeddings produced by the SSR-Encoder contain information only from the selected valid regions of the image.


% When it is difficult to distinguish multiple concepts existing on an image by using text description, it is difficult to generate certain concepts by using text query input. For example, if there are two people in an image, it is not possible to use "people" to select one of them. To solve this problem, we support another query modality input: mask. 

\begin{figure*}[!h]
\centering
\vspace{-0.5cm}
\includegraphics[width=0.88\textwidth]{images/images_01.jpg}
    \caption{\textbf{Qualitative results} of \textbf{SSR-Encoder} in different generative capabilities.}
    \label{image1}
\end{figure*}

\subsection{Subject Conditioned Generation}
\label{sec:3.3}

%The SSR-Ecoder is capable of generating multiscale subject embedding $E_S$. Then the $E_S$ can be used as a new condition to guide stable diffusion generation process as Equ.\ref{denoising}.
% The SSR-Encoder is adept at generating multi-scale subject embeddings $E_S$, which can be integrated as a novel conditioning factor in the stable diffusion generation process, as denoted in Equ.\ref{denoising}.


% \begin{equation}
% \eta_\theta\left(z_t, t, E_T, E_{S}\right)
% \label{denoising}
% \end{equation}

%In this work, we choose to project $E_S$ into the cross-attention layers in U-Net, via parallel subject cross-attention modules. To be more specific, for each cross-attention layer of the original U-Net, we build trainable copies of them. The newly added cross attention layers take subject embeddings $E_S$ as input, instead of text embedding $E_T$. This setup is inspired by\cite{ye2023ip,customdiffusion, controlnet}, which exploits trainable copy to best maintain the capability of the original model and trains the KV projection matrices in the U-Net cross-attention layer for image conditioned generation. With the modification, each cross attention layer in UNet then becomes text and subject jointly conditioned. The output value $\mathbf{O}$ of the attention layer now becomes:
In our approach, $\mathbf{E_S}$ is strategically projected into the cross-attention layers of the U-Net. This is achieved through newly added parallel subject cross-attention layers, each corresponding to a cross-attention layer in the original U-Net. Rather than transforming the editing text embedding $\mathbf{E^e_T}$, these new layers are learned for the subject embeddings $\mathbf{E_S}$. Inspired by works like \cite{ye2023ip,customdiffusion, controlnet}, we employ trainable copies of the vanilla cross-attention layers to preserve the efficacy of the original model. These layers are then adapted to train the key and value projection layers specifically for subject-conditioned generation. 
To aware both global and local subject representation, we concatenate all $\mathbf{E_S^k}$ at the token dimension before projection, i.e. $\mathbf{E_S^C}=\operatorname{concat}\left( \mathbf{E_S^k}, \operatorname{dim}=0\right)$, where $\mathbf{E_S^k}\in \mathbb{R}^{N_t\times D_i}$ represents subject representation at the scale of $k$.
The output value $\mathbf{O}$ of the attention layer is formulated as follows:


% \begin{equation}
% \begin{split}
% \mathbf{O}
% &=\underbrace{\operatorname{Softmax}\left(\frac{\mathbf{Q} (\mathbf{W^K}E_T)^{\top}}{\sqrt{d}}\right) \mathbf{W^V}(E_T)}_{\textrm{text condition}} \\
% &+\lambda\underbrace{\sum_{i=0}^K \operatorname{Softmax}\left(\frac{\mathbf{Q} (\mathbf{W^{K}_{(i)}}^{\prime}E^{(i)_S)^{\top}}{\sqrt{d}}\right) \mathbf{W^V_i}^{\prime} E^i_S}_{\textrm{subject condition}}
% \end{split}
% \end{equation}
\begin{equation}
\begin{split}
\mathbf{O}
&=\underbrace{\operatorname{CrossAttntion}\left(\mathbf{Q}, \mathbf{K}, \mathbf{V}, \mathbf{E^e_T}, \mathbf{z_t}\right)}_{\textrm{text condition}} \\
&+\lambda\underbrace{\operatorname{CrossAttntion}\left(\mathbf{Q}, \mathbf{K_{S}}, \mathbf{V_{S}}, \mathbf{E_S^{C}}, \mathbf{z_t}\right)}_{\textrm{subject condition}}
\end{split}
\end{equation}
where %$\mathbf{Q}$ is latent features in U-Net, $\mathbf{W_K}$, $\mathbf{W_V}$ are the key, and values projection matrices that capture text condition $E_T$, and $\mathbf{\widehat{W_K}}$, $\mathbf{\widehat{W_V}}$ are the trainable copies of respective projection matrices that capture subject condition $E_S$. $\lambda$ is a hyperparameter that balances the strength of the subject condition, the default value is set to $1$. 
$\mathbf{E^e_T}$ represents the editing text embedding and $\mathbf{z_t}$ represents the U-Net embeddings.
$\mathbf{Q}, \mathbf{K}, \mathbf{V}$ represents query, key and value projection layers in original text branch respectively while $\mathbf{K_{S}}, \mathbf{V_{S}}$ represents trainable copies of key and value projection layers for concatenated subject embedding $\mathbf{E_S^{C}}$.

By our subject conditioned generation, text-to-image diffusion models can generate target subject conditioned on both editing text embeddings and subject embeddings.

\subsection{Model Training and Inference}
\label{sec:3.4}
%During training, we take each image and its paired text from multimodal datasets as inputs, with the input image itself regarded as the ground truth. The trainable parameters include the Token-to-Patch Aligner and the subject cross-attention modules. 
During the training phase, our model processes paired images and texts from multimodal datasets. The trainable components include the Token-to-Patch Aligner and the subject cross-attention layers.

%Unlike CLIP that aligns global image features and global text features, Token-to-Patch Aligner requires fine-grained token-to-patch alignment. We devise an embedding regularization loss to fulfill this requirement. Specifically, we regularize the subject embeddings $E_S$ to be similar to the corresponding text token $E_T$. The loss term is calculated via cosine similarity function as Equ.\ref{equ:reg}:
In contrast to CLIP, which aligns global image features with global text features, our token-to-patch Aligner demands a more granular token-to-patch alignment. To achieve this, we employ an embedding regularization loss. This loss encourages similarity between the subject embeddings $\mathbf{E_S}$ and the corresponding query text tokens $\mathbf{E^q_T}$, using a cosine similarity function as detailed in Equ.\ref{equ:reg}:

\begin{equation}
\mathbf{\overline{E_{S}}} = \operatorname{Mean}\left(
\mathbf{E_{S}^0}, \mathbf{E_{S}^1}, ..., \mathbf{E_{S}^K} \right)
\end{equation}
\begin{equation}
\begin{split}
\mathcal{L}_{reg} = \operatorname{CosineSim} \left(\mathbf{\overline{E_{S}}}, \mathbf{E^q_T}\right) = 1 - \frac{\mathbf{\overline{E_{S}}} \cdot \mathbf{E^q_T}}{|\mathbf{\overline{E_{S}}}||\mathbf{E^q_T}|}
\end{split}
\label{equ:reg}
\end{equation}
where $\overline{\mathbf{E_{S}}}$ is the mean of subject embeddings and $\mathbf{E^q_{T}}$ is the query text embeddings. 
As demonstrated in Fig.\ref{image8}, our T2I Aligner, trained on a large scale of image-text pairs, can effectively match text and image regions. This capability is a key aspect of selective subject-driven generation.

Similar to the original Stable diffusion model, our training objective also includes the same $\mathcal{L}_{LDM}$ loss, as outlined in Equ.\ref{equ:simple}:
\begin{equation}
\mathcal{L}_{LDM}(\bm{\theta})=\mathbb{E}_{\mathbf{z_0}, t, \bm{\eta}}\left[\left\|\bm{\eta}-\bm{\eta_\theta}\left(\mathbf{z_t}, t, \mathbf{E^e_T}, \mathbf{E_{S}}\right)\right\|_2^2\right]
\label{equ:simple}
\end{equation}
where $\mathbf{z_t}$ is the latent noisy image at time step $t$ obtained from the training images, $\bm{\eta}$ is the latent noise ground-truth. $\bm{\eta_\theta}$ is the noise prediction model with parameters $\bm{\theta}$. $\mathbf{E_{S}}$ is SSR-Encoder's output.

% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.48\textwidth]{images/images_02_2.jpg}
%     \caption{Results of selective concept-guided image generation from multiple images.}
%     \label{image2}
% \end{figure}

%\textbf{Embedding Regularization Loss.} Training the model with only the reconstruction loss function can easily lead to overfitting and cause the Layered Cross-Attention Module to lose its text-image align capability as shown in Fig\ref{image4} (the 4-th column). To keep the Selected Image Embedding $E_{S}$ within the domain of CLIP's text embeddings and prevent the model from overfitting, we use the cosine similarity loss function between the SSR-Encoder output's Selected Image Embeddings $E_{S}$ and the text embeddings $E_{t}$ as regularization loss. This loss function can be expressed as:
% \begin{equation}
% \mathbf{\overline{E_{S}}} = \operatorname{mean}\left(
% E_{S}^1, E_{S}^2, ..., E_{S}^6 \right)
% \end{equation}
% \begin{equation}
% \begin{split}
% \mathcal{L}_{reg} = \operatorname{CosineSim} \left(\mathbf{\overline{E_{S}}}, \mathbf{E_t}\right) = 1 - \frac{\mathbf{\overline{E_{S}}} \cdot E_t}{|\mathbf{\overline{E_{S}}}||\mathbf{E_t}|}
% \end{split}
% \end{equation}
% where $E_{S}$ is the mean of Selected Image Embeddings from 6 scales and $E_{t}$ is the text embeddings.

Thus, our total loss function is formulated as:
\begin{equation}
\mathcal{L}_{total}=\mathcal{L}_{LDM} + \tau \mathcal{L}_{reg}
\end{equation}
where $\tau$ %is a constant setting to 0.01.As shown in Fig\ref{image4} (last column) the addition of $\mathcal{L}_{reg}$ to the loss succeeds in ensuring SSR-Encoder's text-image align capability and generates images that are consistent with the concept prompt and the reference image.
is set as a constant, with a value of 0.01. This setting balances the contributions of the two losses. As depicted in Fig.\ref{image4} (in the last column), the inclusion of $\mathcal{L}_{reg}$ significantly enhances the text-image alignment capabilities of the SSR-Encoder. This improvement is evident in the generated images, which consistently align with both the subject prompt and the details of the reference image.

During inference, our method has the ability to decompose different subjects from a single image, and further, we extend the single image input to multiple image input and perform a separate forward calculation for each image in our SSR-Encoder. By simply concat outputs together to feed into U-Net, we are able to combine the constituent parts of multiple scenes together.


==> sec/3_2_method_prev.tex <==

\begin{table}[ht]
\centering
\scriptsize % 设置字体为非常小
\begin{tabular}{c c} % 移除两端的竖线
\hline
\textbf{Encoder} & \textbf{ID-preserving method} \\ \hline
CLIP image encoder & IP-Adapter, IP-Adapter Plus, Photomaker, Face0 \\ \hline
Arcface encoder & InstantID, Photomaker v2, PuLID, IP-Adapter-FaceID \\ \hline
CLIP \& Arcface encoder & IDAdapter,  Storymaker \\ \hline
\end{tabular}
\caption{Overview of Encoder-Based Methods for ID Preservation}
\end{table}



\section{Problem Definition}
We consider two participants in the scenario of using reference-based methods: "image protector" Alice and "image exploiter" Bob. Bob customizes content by exploiting Alice's photos shared on social media, using encoder-based ID-preserving methods, while Alice aims to protect her images by adding adversarial noise to thwart Bob's methods, inducing distortions or significant decreases in ID similarity in the generated content. Specifically, we explain the workflow of the two parties as follows:

\textbf{Image Protector Alice:} The image protector aims to provide protection for images against exploitation by encoder-based ID-preserving methods. In this context, the chosen protection method involves adding imperceptible protective perturbations to the images, with the goal of providing protection while minimizing modifications to the original image. In real-world scenarios, the image protector often faces challenges, as there are numerous encoder-based ID-preserving methods.

\textbf{Image Exploiter Bob:} Bob aims to use images collected from the internet for ID-consistent image generation. Bob can choose any encoder-based ID-preserving method, which requires the image protector's protective measures to be universally applicable. Protected images may undergo natural disturbances such as cropping, JEPG compression, and blurring.

\textbf{Objective of the Study:}  Given an image $x$ containing a face portrait, our objective is to generate adversarial perturbations $\delta$ that protect against ID-preserving generation. We aim to maximize the difference in identity consistency between the unperturbed generated image $g(x)$ and the perturbed generated image $g(x+\delta)$, where $g$ is an ID-preserving generator. To achieve this, we optimize a noise encoder network $E_\theta$ by solving:
\begin{equation}
    \min_\theta S
    \left\{
        g(x), g(x+\delta)
    \right\}, \quad \delta = E_\theta(x)
\end{equation}
\noindent subject to the constraint $\lVert \delta \rVert_\infty < \epsilon$. Here, $S$ denotes an identity similarity metric, which we evaluate using ArcFace and CLIP similarities, supplemented by a qualitative user study.

% The objective of this paper is to add imperceptible adversarial noise to images, formalized as \( I_{\text{adv}} = I + \text{noise} \), where \( I \) and \( I_{\text{adv}} \) represent the original and protected images, respectively. These images serve as inputs to customization methods, and the outputs \( \text{Gen}(I) \) and \( \text{Gen}(I_{\text{adv}}) \) are compared. If \( \text{Gen}(I_{\text{adv}}) \) exhibits clear deviations in identity or noticeable distortions, the protection is considered successful.



% \textbf{Single Method Attack}
% This refers to the addition of adversarial noise to an image targeting a specific method. The proposed approach in this paper demonstrates effective attacks on all currently open-source available ID Preservation methods, such as Instant-ID, Photomaker, and IP-Adapter.

% \textbf{Joint Attack}
% A joint attack involves adding adversarial noise (in a single noise addition) and simultaneously targeting multiple ID-Preserving methods.


% \subsection{问题定义}
%我们考虑到两个参与者在使用reference-absed方法的情况：“图像保护者”Alice 和“图像利用者”Bob。Bob通过利用Alice在社交媒体上发布的照片，使用被Encoder-based ID-preserving方法定制内容，而Alice希望通过添加对抗性噪声来保护她的图像，阻断Bob的方法，以在生成的内容中诱发失真或者明显的ID相似度下降。

% 具体来说，我们解释这两方的工作流程如下：

% \textbf{图像保护者Alice：}图像保护者旨在为图像提供保护，防止被Encoder-based ID-preserving方法利用。在这种情境中，选择的保护方法包括向图像添加不易察觉的保护性扰动，目标是在尽量减少对原始图像的修改的同时提供保护。在真实世界的情境中，图像保护者常面临挑战，因为Encoder-based ID-preserving方法众多。

% \textbf{图像利用者Bob：}Bob旨在使用从互联网上收集的图像用于ID一致性的图像生成。Bob可以选择任何Encoder-based ID-preserving方法，这要求图像保护者的保护措施是广泛通用的。 受保护的图像可能会经历剪裁、压缩和模糊等自然干扰。

% 本文的目标是将不易察觉的对抗性噪声添加到图像中，形式化为\( I' = I + \text{noise} \)，其中\( I \)和\( I' \)分别代表原始图像和被保护图像。这些图像作为客制化方法的输入，这些方法的输出\( O \)和\( O' \)将进行比较。\( O' \) 中的人物身份明显出现偏差或出现明显的失真则表明保护成功。

% \section{Problem}
% \subsection{Background}
% \textbf{Adversarial attacks.} The goal of adversarial attacks is to find an imperceptible perturbation of an input image to mislead the behavior of given models. Typical works have been developed for classification problems where for a model \(f\), an adversarial example \(x'\) of an input image \(x\) is generated to stay visually undetectable while inducing a misclassification \(y_{\text{true}} \neq f(x')\) (untargeted attack), or making the model predict a predefined target label \(y_{\text{target}} = f(x_{\text{adv}}) \neq y_{\text{true}}\) (targeted attack). The minimal visual difference is usually enforced by bounding the perturbation to be within an epsilon-ball, that is \(\|x' - x\|_p < \eta\). To achieve this objective, denoting \(\Delta = \{\delta : \|\delta\|_p \leq \eta\}\), we find the optimal perturbation \(\delta\) to maximize the classification loss in the untargeted version:
% \[
% \delta_{\text{adv}} = \arg\max_{\delta \in \Delta} L(f(x + \delta), y_{\text{true}})
% \]
% or to minimize the loss for the targeted variant:
% \[
% \delta_{\text{adv}} = \arg\min_{\delta \in \Delta} L(f(x + \delta), y_{\text{target}})
% \]
% Projected Gradient Descent (PGD) [36] is a commonly used attack based on an iterative optimization process. The updating pipeline to predict \(x'\) for untargeted attack is:
% \[
% \begin{aligned}
%     x'_0 &= x \\
%     x'_k &= \Pi_{(x, \eta)}(x'_{k-1} + \alpha \cdot \text{sgn}(\nabla_x L(f(x'_{k-1}), y_{\text{true}})))
% \end{aligned}
% \]
% where \(\Pi_{(x, \eta)}(z)\) restrains pixel values of \(z\) within an \(\eta\)-ball around the original values in \(x\). We acquire the adversarial example \(x'\) after a pre-defined number of iterations.

% \textbf{Encoder-based ID-Preserving methods.}
%  To ease the resource demand necessitated by online tuning, a series of tuning-free methods [36, 38, 25, 42, 20, 41, 3] have emerged, which directly encode ID information into the generation process. The major challenge these methods encounter is minimizing disruption to the original behavior of T2I models while still maintaining high ID fidelity. In terms of minimizing the disruption, one plausible approach is to utilize a face recognition model[4] to extract more abstract and relevant facial domain-specific representations, as done by InstantID and PuLID. 

% \subsection{Problem Definition.}
% % Bob uses Encoder-based ID-Preserving Methods to illicitly extract others' identity information, generating unauthorized counterfeit images. Alice wishes to post her own photos on social media and needs to add adversarial noise to the images to protect her identity information.

% Bob collected photos containing Alice's face portrait and used them for Encoder-based ID-preserving generation to generate counterfeit photos of Alice. To protect her photos (e.g. posted on social media) from being misused as such, Alice wishes to add adversarial perturbations on her face portraits.

% The objective of this paper is to add imperceptible adversarial noise to facial images, formulated as \( I' = I + \text{noise} \), where \( I \) and \( I' \) represent the original and the attacked images, respectively. These images serve as inputs to Encoder-based ID Preservation Methods, and the outputs of these methods, \( O \) and \( O' \), are compared. A significant decrease in identity consistency between \( O \) and \( O' \) indicates a successful attack. For assessing identity consistency, we use Arcface similarity and CLIP similarity as quantitative metrics, complemented by a user study for qualitative evaluation.

% % >>>>>>>>>>Sam>>>>>>>>>>

% Given an image $x$ containing a face portrait, our objective is to generate adversarial perturbations $\delta$ that protect against ID-preserving generation. We aim to maximize the difference in identity consistency between the unperturbed generated image $g(x)$ and the perturbed generated image $g(x+\delta)$, where $g$ is an ID-preserving generator. To achieve this, we optimize a noise encoder network $E_\theta$ by solving:

% \begin{equation}
%     \min_\theta S
%     \left\{
%         g(x), g(x+\delta)
%     \right\}, \quad \delta = E_\theta(x)
% \end{equation}

% \noindent subject to the constraint $\lVert \delta \rVert_\infty < \epsilon$. Here, $S$ denotes an identity similarity metric, which we evaluate using ArcFace and CLIP similarities, supplemented by a qualitative user study.

% % <<<<<<<<<<Sam<<<<<<<<<<

% \textbf{Single Method Attack}
% This refers to the addition of adversarial noise to an image targeting a specific method. The proposed approach in this paper demonstrates effective attacks on all currently open-source available ID Preservation methods, such as Instant-ID, Photomaker, and IP-Adapter.

% \textbf{Joint Attack}
% A joint attack involves adding adversarial noise (in a single noise addition) and simultaneously targeting multiple ID-Preserving methods.


\section{Method}
In Section 4.1, we first introduce the overall method. In Section 4.2, we discuss the Noise Encoder in detail. In Section 4.3, we describe joint optimization using PGD. In Section 4.4, we introduce the design of our loss function. In Section 4.5, we explain the development of Adaptive Attacks to enhance robustness.

% 在4.1节，我们首先介绍介绍整体方法 在4.2节，我们介绍噪声encoder， 在4.3节，介绍通过pgd联合优化， 在4.4节， 我们介绍损失函数设计，  在4.5节，介绍为了提升鲁棒性提出的Adaptive Attacks。


\subsection{Overall Method}
This section introduces the overall framework of our method, as illustrated in Figure 2. Our approach consists of several key components: the Noise Encoder, loss function design, PGD joint optimization, and Adaptive Attacks. The Noise Encoder adds adversarial noise to the image, forming the protected image \(I_{\text{adv}}\). We optimize the noise addition through a meticulously designed loss function that maximizes the difference in the image features in both ArcFace and CLIP feature spaces before and after noise addition, ensuring effective image protection. For training, the adversarial noise can be directly optimized on individual images using PGD, or the Noise Encoder can be trained on large datasets to predict adversarial noise.

% 本节介绍方法的整体框架，如图2所示，我们的方法可以分为几个关键部分：Noise Encoder，损失函数设计，PGD联合优化，和Adaptive attacks. Noise Encoder给图像添加对抗噪声,形成被保护图像x_{adv}。我们通过精心设计的损失函数，最大化添加噪声前后图像在Arcface特征空间和CLIP 特征空间的差异，实现图像保护。训练方面， 可以在单张图像上直接通过PGD优化对抗噪声， 也可以在海量数据上训练Noise encoder预测对抗噪声。






% \subsection{Noise Encoder}
% % 我们的目标是输入需要保护的图像，Noise Encoder通过前向过程生成与图像相同尺寸的对抗噪声。在设计Noise Encoder的结构时，我们曾尝试了Hidden提出的隐水印嵌入方法以及Stable Diffusion的U-Net结构，但效果都不理想。最终，我们基于DiT结构提出了本文的Noise Encoder。DiT是一种基于transformers的新型扩散模型，称为Diffusion Transformers，遵循Vision Transformers（ViTs）的最佳实践。ViTs在视觉识别任务中的扩展性已被证明优于传统卷积网络（如ResNet）。具体来说，DiT模型通过将输入图像进行patch化，将图像划分为多个小块，并将这些块作为transformers的输入序列。经过多层transformer block处理后，逐步去噪，最终生成高质量的图像。

% % 在我们的Noise Encoder设计中，和DiT中的设计有如下不同，1.我们的Noise Encoder通过单次推理得到对抗噪声而非迭代去噪 2. 我们移除了DiT中与扩散过程相关的额外条件信息，如噪声时间步长t、类别标签c和自然语言等。3. DiT在VAE的隐空间去噪，而本文方法在像素域预测对抗噪声， 输入的通道数和分辨率不同。考虑到本文攻击的定制化方法普遍使用SD1.5作为基础模型，ReferenceNet的输入图像分辨率和去噪U-Net的分辨率通常设置为512×512，因此我们将DiT的训练分辨率也设置为512×512，以确保与这些定制化生成任务的兼容性和攻击效果。 
% % 为了确保对抗噪声在各种图像处理条件下仍然有效，我们在使用带噪图像 \( I' \)之前，应用一系列数据增强。这些增强包括可微分的裁剪、调整大小、JPEG 压缩和颜色调整，这有助于保持对抗噪声在常见图像变换下的鲁棒性。

% Our objective is to input an image that needs protection, and the Noise Encoder generates adversarial noise of the same size as the image through a forward process. In designing the structure of the noise encoder, we initially tried the hidden watermark embedding method proposed by Hidden and the U-Net structure from stable diffusion, but neither yielded satisfactory results. Ultimately, we proposed the Noise Encoder based on the DiT structure. DiT, a new diffusion model based on transformers, is referred to as Diffusion Transformers and follows the best practices of Vision Transformers (ViTs). ViTs have demonstrated superior scalability in visual recognition tasks compared to traditional convolutional networks like ResNet. Specifically, the DiT model processes input images by patchifying them into smaller blocks, which are then fed as input sequences into transformers. After being processed by multiple transformer blocks, the noise is gradually removed, resulting in high-quality image generation.

% In our Noise Encoder design, there are several key differences from the DiT design: 1. Our Noise Encoder generates adversarial noise in a single inference rather than iterative denoising. 2. We removed the additional conditional information related to the diffusion process from DiT, such as noise timesteps t, class labels c, and natural language. 3. DiT performs denoising in the latent space of the VAE, whereas our method predicts adversarial noise in the pixel domain, with differences in input channels and resolution. Considering that the customization methods targeted by our attacks typically use SD1.5 as the base model, with the input image resolution for ReferenceNet and the denoising U-Net set to 512×512, we also set the training resolution of DiT to 512×512 to ensure compatibility with these customized generation tasks and to enhance the effectiveness of the attack.

% To ensure the adversarial noise retains its effectiveness under various image processing conditions, we apply a series of data augmentations before utilizing the noised image \( I' \). These augmentations include differentiable cropping, resizing, JPEG compression, and color adjustments, all of which help maintain the robustness of the adversarial noise against common image transformations.


\subsection{Noise Encoder}
This section introduces the Noise Encoder used in ID-Protector. In designing the structure of the noise encoder, we initially tried the hidden watermark embedding method proposed by Hidden and the U-Net structure from stable diffusion, but neither yielded satisfactory results. Ultimately, we proposed the Noise Encoder based on the DiT structure. DiT, a new diffusion model based on transformers, is referred to as Diffusion Transformers and follows the best practices of Vision Transformers (ViTs). ViTs have demonstrated superior scalability in visual recognition tasks compared to traditional convolutional networks like ResNet. We employ a DIT structure with an input resolution of \( 224 \times 224 \). A three-channel image is input, and facial regions are detected using a face detector. The detected face region, represented as a mask, serves as the fourth channel merged with the input image for the Noise Encoder. This approach aims to reduce the learning difficulty of the network, as attacks for InstantID need to focus on facial regions. To make the adversarial noise less perceptible, the output of the Noise Encoder is constrained within a range of \(\pm 0.1\).

% >>>>>>>>>>Sam>>>>>>>>>>
 % - DiT input with CLIP preprocessing
 % - Architecture design: 4 channel input, 3 channel rgb output, conditional branches removed
 % - One-hot arcface prior design: additional channel indicating face alignment region; make it easier to train; otherwise network may need to inherit face localisation capabilities from InsightFace
 % - Output regularised to within [-1, 1], scaled to [-\epsilon, epsilon] before perturbing

We used the DiT architecture as the adversarial noise encoder for ID-Protector, and removed the conditional branches injecting timesteps and context. The network has a 4-channel $224\times 224$ input, including three RGB image channels and an additional one-hot channel for a face alignment prior. The one-hot prior channel marks the facial regions within the input for the InstantID pipeline. This can reduce the difficulty of the network's learning task, as the network would otherwise need to learn the face alignment process for InstantID simultaneously. The network outputs three-channel adversarial perturbations with a range of $[-1, 1]$, which can be scaled to $[-\epsilon, \epsilon]$ and added to the RGB image.

% 本节介绍了 ID-Protector 中使用的噪声编码器。在设计Noise Encoder的结构时，我们曾尝试了Hidden提出的隐水印嵌入方法以及Stable Diffusion的U-Net结构，但效果都不理想。最终，我们基于DiT结构提出了本文的Noise Encoder。DiT是一种基于transformers的新型扩散模型，称为Diffusion Transformers，遵循Vision Transformers（ViTs）的最佳实践。ViTs在视觉识别任务中的扩展性已被证明优于传统卷积网络（如ResNet）。 我们使用具有 \(224 \times 224\) 输入分辨率的 DIT 结构。输入为三通道图像，并使用面部检测器检测面部区域。检测到的面部区域被表示为一个掩码，作为第四通道与输入图像合并到噪声编码器中。这种方法旨在降低网络的学习难度，因为 InstantID 的攻击需要集中在面部区域。为了使对抗性噪声不易被察觉，噪声编码器的输出被限制在 \(\pm 0.1\) 范围内。

% 我们使用 DiT 架构作为 ID-Protector 的对抗性噪声编码器，并移除了注入时间步和上下文的条件分支。网络有一个包括三个 RGB 图像通道和一个额外的 one-hot 面部对齐先验通道的 4 通道 \(224\times 224\) 输入。One-hot 先验通道在输入中标记 InstantID 管道的面部区域。这可以减少网络学习任务的难度，否则网络需要同时学习 InstantID 的面部对齐过程。网络输出三通道的对抗性扰动，范围为 \([-1, 1]\)，可以缩放到 \([- \epsilon, \epsilon]\) 并加到 RGB 图像上。


% <<<<<<<<<<Sam<<<<<<<<<<


\subsection{PGD Joint Optimization}
We introduce our Anti-Reference (PGD) method, where adversarial noise is optimized directly using PGD (Projected Gradient Descent). PGD iteratively perturbs the input image \(I\) within a predefined bound, ensuring the noise remains imperceptible while maximizing its impact on the model’s predictions. Unlike the Noise Encoder, which generates noise in a single pass, PGD updates the noise iteratively by calculating the gradient of the loss function with respect to the image. At each iteration, the adversarial noise is updated as:

\[
I_{adv}^{(k+1)} = \Pi_{I + \epsilon} \left( I_{adv}^{(k)} + \alpha \cdot \text{sign} \left( \nabla_{I_{adv}^{(k)}} L_{\text{total}} \right) \right)
\]

Here, \(I_{adv}^{(k)}\) is the adversarial image at iteration \(k\), \(\alpha\) is the step size, and \(\epsilon\) defines the perturbation bound. The projection \(\Pi_{I + \epsilon}\) ensures the noise stays within the allowed limits.

By optimizing both \(L_{\text{adv}}\) and \(L_{\text{con\_adv}}\), PGD effectively disrupts both the diffusion process and conditional adversarial predictions. Our experiments show that PGD provides strong protection across various reference-based customization methods, with gradually increasing noise impact while preserving image quality. Although Noise Encoder generates noise faster, PGD's iterative process delivers stronger protection across tasks, albeit with higher computational costs, making it suitable for scenarios requiring maximum protection.

% \subsection{PGD联合优化}

% 我们介绍了Anti-Reference (PGD) 方法，在该方法中，使用PGD（投影梯度下降）直接优化对抗噪声。PGD在预定义的范围内迭代地扰动输入图像\(I\)，确保噪声保持不可察觉的同时，最大化其对模型预测的影响。
% 与一次性生成噪声的Noise Encoder不同，PGD通过计算损失函数相对于图像的梯度来迭代更新噪声。在每次迭代中，对抗噪声的更新公式为：

% \[
% I_{adv}^{(k+1)} = \Pi_{I + \epsilon} \left( I_{adv}^{(k)} + \alpha \cdot \text{sign} \left( \nabla_{I_{adv}^{(k)}} L_{\text{total}} \right) \right)
% \]

% 其中，\(I_{adv}^{(k)}\)为第\(k\)次迭代的对抗图像，\(\alpha\)为步长，\(\epsilon\)为扰动范围的限制。投影操作\(\Pi_{I + \epsilon}\)确保噪声保持在允许的范围内。

% 通过优化\(L_{\text{adv}}\)和\(L_{\text{con\_adv}}\)，PGD有效地破坏了扩散过程和条件对抗预测。我们的实验表明，PGD在各种参考驱动的定制生成方法中提供了强大的保护，随着噪声的逐步增加，仍然能保持图像质量。
% 图6展示了PGD优化的噪声与Noise Encoder的比较。虽然Noise Encoder生成噪声的速度更快，但PGD的迭代过程在各个任务中提供了更强的保护，尽管计算开销更高。PGD的联合优化在效率和鲁棒性之间提供了平衡，特别适合需要最大保护的场景。

\subsection{Loss Function}
The design of the loss function is a key aspect of ID-Protector. This section describes different loss functions used for various ID preservation methods. The paper implements attacks on four common methods: InstantID, IP-Adapter, IP-Adapter Plus, and PhotoMaker. The loss functions are defined as follows for each method:


% InstantID使用预训练的Arcface encoder作为编码器，提取人脸embedding，在此之后，人脸的embedding将作为Ip- adapter分支和IdentityNet分支的输入，作为text2image的条件。因此，只要成功攻击Arcface encoder即可攻击InstantID。 损失函数被定义为加对抗噪声前后人脸embedding的余弦损失

\textbf{InstantID} InstantID uses a pre-trained Arcface encoder as the feature extractor to obtain face embeddings. These embeddings are then used as inputs for both the IP-Adapter branch and the IdentityNet branch, serving as conditions for text-to-image generation. Therefore, successfully attacking the Arcface encoder is sufficient to attack InstantID. The loss function is defined as the cosine loss between the face embeddings before and after adding the adversarial noise.

The loss function can be expressed  as:

\[
L_{\text{cos}} = 1 - \frac{\mathbf{e}_1 \cdot \mathbf{e}_2}{\|\mathbf{e}_1\| \|\mathbf{e}_2\|}
\]

where \(\mathbf{e}_1\) and \(\mathbf{e}_2\) represent the face embeddings before and after adding adversarial noise, respectively.

% IP-Adapter 使用CLIP image encoder作为图像编码器，输出特征e维度为1*768，这个特征在经过Adapter模块后作为扩散模型的额外条件，因此只要成功攻击e即可攻击IP-Adapter。损失函数被定义为加对抗噪声前后CLIP image embedding的余弦损失。

\textbf{IP-Adapter}
IP-Adapter uses a CLIP image encoder as the image encoder, producing features \(\mathbf{e}\) with a dimension of \(1 \times 768\). This feature is used as an additional condition for the diffusion model after passing through the Adapter module. Therefore, successfully attacking \(\mathbf{e}\) is sufficient to attack IP-Adapter. The loss function is defined as the cosine loss between the CLIP image embeddings before and after adding the adversarial noise.

The loss function is given by:

\[
L_{\text{cos}} = 1 - \frac{\mathbf{e}_1 \cdot \mathbf{e}_2}{\|\mathbf{e}_1\| \|\mathbf{e}_2\|}
\]

where \(\mathbf{e}_1\) and \(\mathbf{e}_2\) represent the CLIP image embeddings before and after adding adversarial noise, respectively.

% IP-Adapter Plus同样使用CLIP image encoder作为图像编码器，不同之处在于使用的是projection层之前的patch特征e’维度为257*1280，这个特征在经过Adapter模块后作为扩散模型的额外条件，因此只要成功攻击e'即可攻击IP-Adapter plus。损失函数被定义为加对抗噪声前后patch CLIP image embedding的余弦损失。
\textbf{IP-Adapter Plus} IP-Adapter Plus also uses a CLIP image encoder as the image encoder. The difference is that it uses the patch features \(\mathbf{e}'\) with a dimension of \(257 \times 1280\) before the projection layer. This feature, after passing through the Adapter module, serves as an additional condition for the diffusion model. Therefore, successfully attacking \(\mathbf{e}'\) is sufficient to attack IP-Adapter Plus. The loss function is defined as the cosine loss between the patch CLIP image embeddings before and after adding the adversarial noise.

The loss function is given by:

\[
L_{\text{cos}} = 1 - \frac{\mathbf{e}'_1 \cdot \mathbf{e}'_2}{\|\mathbf{e}'_1\| \|\mathbf{e}'_2\|}
\]

where \(\mathbf{e}'_1\) and \(\mathbf{e}'_2\) represent the patch CLIP image embeddings before and after adding adversarial noise, respectively.


\textbf{Photomaker} Photomaker also uses a CLIP image encoder as the image encoder. The difference is that it uses the patch features \(\mathbf{e}'\) with a dimension of \(257 \times 1280\) before the projection layer. This feature, after passing through the Adapter module, serves as an additional condition for the diffusion model. Therefore, successfully attacking \(\mathbf{e}'\) is sufficient to attack Photomaker. The loss function is defined as the cosine loss between the patch CLIP image embeddings before and after adding the adversarial noise.

The loss function is given by:

\[
L_{\text{cos}} = 1 - \frac{\mathbf{e}'_1 \cdot \mathbf{e}'_2}{\|\mathbf{e}'_1\| \|\mathbf{e}'_2\|}
\]

where \(\mathbf{e}'_1\) and \(\mathbf{e}'_2\) represent the patch CLIP image embeddings before and after adding adversarial noise, respectively.


\textbf{Image Regularization Loss}  To make the adversarial noise less perceptible, we calculate the Mean Squared Error (MSE) of the images before and after noise addition as the regularization loss.

\[
L_{\text{reg}} = \mathbb{E}_{x} \left[ \| x - (x + \delta) \|^2 \right]
\]


\textbf{Total Loss} For joint attacks, a weighted loss is employed, with weights adjusted experimentally to balance the reduction across all four losses, achieving balanced attack performance across all tasks.
\[
\ L_{total} = W_1 \cdot L_1 + W_2 \cdot L_2 + W_3 \cdot L_3 + W_4 \cdot L_4 + W_5 \cdot L_r
\]


% \subsection{Differentiable Preprocessing and Perturbation}
% This paper implements attacks on the four common ID preservation methods mentioned earlier. Since InstantID uses the Arcface encoder, which differs from the other methods that use the CLIP Image encoder, the preprocessing of the input images also varies. In fact, for a photo, the Arcface encoder in InstantID first detects the face frame and then performs crop \& refine on this detected face frame. Therefore, the adversarial noise will also undergo crop \& refine, causing a truncation of gradients. To address this, we have implemented a differentiable crop \& refine.

% \subsection{Adaptive Data Augmentation}
% We aim for the adversarial noise to be robust against common image enhancement techniques to protect the image. Therefore, before sending the noised image \( I' \) to the Noise Encoder, we perform data augmentations on \( I' \). These augmentations include cropping, resizing, JPEG compression, and color transformations.

% >>>>>>>>>>Sam>>>>>>>>>>

\subsection*{Training}

...


\subsection{Adaptive Attacks}

\textbf{Robustness against distortions.} Since InstantID uses the Arcface encoder, which differs from the other methods that use the CLIP Image encoder, the preprocessing of the input images also varies. In fact, for a photo, the Arcface encoder in InstantID first detects the face frame and then performs crop \& refine on this detected face frame.  To ensure ID protection remains effective even with image distortions, we apply data augmentation to the adversarial examples ($x_\text{adv} = x+\delta$) during training, before using them for IP-preserving generation. The augmentations include JPEG compression, random affine transformations, and interpolation error simulations. 

\textbf{Robustness against InstantID alignment error.} InstantID uses ArcFace to extract facial features, which requires five facial landmarks (eyes, mouth corners, and nose tip) to be as close as possible to predefined locations. InstantID first uses InsightFace to detect these landmarks $\Tilde{p}$ in the image, then applies an affine transformation $\Tilde{p}'=A \Tilde{p}$ to align them with the predefined locations $\Tilde{q}$. The transformation matrix $A$ is obtained by minimizing the least square error between $\Tilde{q}$ and $\Tilde{p}'$. 

We assumed fixed $\Tilde{p}$ during training for clean and adversarial images, so as to reduce computational overhead. However, at inference times, the adversarial perturbations can cause slight shifts in landmark predictions, leading to changes in the fitted affine matrix $A$. This could result in up to 5-pixel deviation in the face input to ArcFace. Without adaptive designs, the misalignment is sufficient to nullify the adversarial perturbations, and the attack would thus fail.

To make adversarial perturbations adaptive to face alignment discrepancies, we introduce errors to the affine matrix $A$. The face alignment step is now given by

\begin{equation}
    \Tilde{p}' = \left( A + N(0, \sigma I)\right) \Tilde{p}.
\end{equation}

We incrementally scan $\sigma$ values. At $\sigma=0.003$, our method successfully attacks InstantID, indicating that this level of randomness covers the gap between noise encoder training and inference. We hence use this value of $\sigma$ during training.

% <<<<<<<<<<Sam<<<<<<<<<<





==> sec/4_experiments_prev.tex <==
\section{Experiment}
\label{sec:exper}

\subsection{Experimental Setup}
% \noindent \textbf{Training data.} This paper aims to protect images containing people, not just cropped faces, therefore we use un-cropped images from the CelebA dataset as the training set.

\noindent \textbf{Training Data.} For practicality, we selected 190,000 uncropped images from the CelebA dataset as the training set. These images have arbitrary sizes and aspect ratios.

% 本文想要实现包含人的图像的保护，而不是仅限于裁切后的人脸，因此使用CelebA裁切前的图像作为训练集。

% \noindent \textbf{Experimental details.} We trained on 200,000 images using four 80GB A100 GPUs, with a batch size of 96 for several epochs, utilizing a learning rate decay strategy. We employed a pre-trained DiT-S/8 model as the Noise Encoder. 

\noindent \textbf{Training Details.} We trained the DiT-S/8 adversarial noise encoder on four 80GB Nvidia H100 GPUs with a batch size of 112, completing the training in 10 days.

% 我们使用4张80G A100, 在20万图像上， batchsize 为96训练了Xepoch, 用了学习率衰减策略。我们使用预训练的DiT-S/8 模型作为Noise encoder的预训练模型。

\noindent \textbf{Baseline methods.} PhotoGuard\cite{photoguard}, AdvDM\cite{advdm}, Anti-Dreambooth\cite{antidreambooth}, ACE\cite{ace}, and SimAC\cite{simac} are used as baselines. We systematically evaluate the protection effectiveness of our method and the baseline methods across four identity-consistency generation tasks: IP-Adapter\cite{ipa}, IP-Adapter-plus\cite{ipa}, Photomaker\cite{photomaker}, and InstantID\cite{instantid}.


% 在 PhotoGuard, AdvDM, Anti-Dreambooth, SimAC, ACE 作为baseline。我们系统性的评估了本文方法和baseline方法在4项身份一致性生成任务上的保护效果， IP-Adapter,  IP-Adapter-plus, Photomaker, InstantID。


\noindent \textbf{Evaluation benchmarks.} In terms of building the evaluation dataset, we divided 100 images from CelebA for testing. We generated a total of 50 images using five different prompts for quantitative assessment.

% 评估数据集的构建方面, 我们从CelebA中划分50张测试集，我们使用5个不同的prompt生成共250张图用于定量评估。 

\noindent \textbf{Evaluation metrics.} Quantitative evaluation is twofold: firstly, we directly compute the similarity between images before and after adding protective noise using CLIP-I similarity and Arcface similarity. Secondly, we assess the differences in the customized generation results before and after adding protective noise. We use widely recognized metrics, FDFR and ISM, to quantify generation quality, where a higher FDFR and a lower ISM indicate better protection effectiveness. Additionally, we employ two general image quality assessment metrics, BRISQUE and CLIP-IQA.

% 定量评估分为两方面，一方面我们直接计算加保护噪声前后两张图像的CLIP-I similarity 和 Arface similarity. 另一方面，我们计算加保护噪声前后，客制化生成结果的差异。我们我们使用广泛使用的FDFR 和 ISM，来量化生成质量，其中较高的FDFR 和较低的 ISM代表更好的保护效果。此外，我们使用2个通用的图像质量评估指标，BRISQUE， 和CLIP-IQA。


\subsection{Comparison with baseline methods}
As shown in Figure 5 and Table 2, baseline methods employing VAE attack and diffusion attack, designed for attacking tuning-based customization or image editing methods, utterly fail to protect against threats from ID-Preserving methods. Our method fills this gap in the field, achieving the best scores across all metrics.

% 如图5和表2所示，采用VAE attack和diffusion attack的baseline 方法，为攻击tuning-based custumiztion或图像编辑方法设计，完全不能保护图像免受 ID-Preserving方法的威胁。而我们的方法填补了这一领域的空白，在在所有指标上都取得了最好的成绩。

\subsection{Noise Encoder or PGD?}
This section presents detailed experimental results for IP-protector (Noise Encoder) and IP-protector (PGD). As illustrated in Figure 6 and Table 3, results optimized via PGD demonstrate more significant effects on attacking ID-preserving methods, with better imperceptibility. IP-protector (Noise Encoder), as the first method to implement ID protection through a forward process, also achieved commendable results. Moreover, the time cost is only a ten-thousandth of the PGD method, allowing practitioners to choose the appropriate method based on the situation.
%本节，我们展示IP-protector(Noise Encoder) 和IP-protector(PGD) 的详细实验结果。从图6和表3可以看出，pgd优化的结果对ID维持方法的攻击效果更加显著，同时不可察觉性更好。IP-protector(Noise Encoder) 作为第一个通过前向过程实现ID保护的方法，也取得了不错的成绩。 同时时间开销仅仅是pgd方法的万分之一。 可以视情况决定实际应用中选择哪种方法。

\subsection{Evaluation of Robustness}
% 本节， 我们详细的评估ID-Protector的鲁棒性， 我们测试了对JEPG 压缩， crop&resize， add noise， 仿射变换的鲁棒性。这些操作是图像传播过程常见的图像变换。仿射变换是人脸检测后的afine tranformation中的必要环节。从表5可以看出， 我们的方法展现出来相当的鲁棒性。


In this section, we systematically evaluate the robustness of ID-Protector, testing its resilience against common image transformations encountered during image propagation. These transformations include JPEG compression, cropping and resizing, noise addition, and affine transformations, which are crucial post-face detection. As demonstrated in Table 5, our method exhibits significant robustness.


\subsection{Transfer and generalization effects}
% 虽然本文的损失函数只为4种Encoder-based IDPreserving 方法设计，由于我们直接攻击CLIP image encoder和Arface encoder，ID-Protector的保护噪声在其他客制化方法上也表现出相当的可迁移性。 图7展示了我们在其他4种客制化方法上的效果，他们是Paint-by-example, Anydoor， IPA-faceID和Midjounery的ref模式.


Although the loss function in this paper was specifically developed for four Encoder-based ID-Preserving methods, the protective noise of ID-Protector shows substantial transferability to other customization methods due to our direct attacks on the CLIP image encoder and the ArcFace encoder. Figure 7 illustrates our method's effectiveness on four other customization methods: Paint-by-example, Anydoor, IPA-faceID, and Midjourney's reference mode.


\subsection{Ablation study.}
% 为了评估各个组件的重要性，我们通过系统地去除它们并观察结果来进行实验。

%当不使用Differentiable Preprocessing and Perturbation，我们的方法对InstantID的攻击显著失效，这是因为对抗噪声对Arcface encoder 输入要求的图像预处理不具有鲁棒性. 当不使用 Adaptive Data Augmentation， 我们的方法的鲁棒性显著下降。

To evaluate the significance of various components, we conducted experiments by systematically removing them and observing the outcomes. When not using Differentiable Preprocessing and Perturbation, our method's attack on InstantID fails significantly because the adversarial noise is not robust to the image preprocessing required for the Arcface encoder. Similarly, when not using Adaptive Data Augmentation, the robustness of our method decreases significantly.



% \subsection{Experimental Setup}
% \textbf{Training data.} Our model utilizes the Celeb-A dataset. 
% %数据集是没有经过裁切的Celeb-A数据集，包含20W张人物照片，包含人物特写，半身，全身等。因此我们的模型可以泛化到各种实际使用场景中。

% \textbf{Implementation details.} 
% %我们在20W张人像照片上训练了我们的模型， 采用学习率衰减策略训练了500epoch。 实验中，我们选取InstantID, IP-Adapter, IP-Adapter plus, PhotoMaker作为被攻击的对象。所有的方法均采用其推荐的默认设置以保证测试的公平性。

% \subsection{Evaluation Metrics}
% %在本节中，我们将呈现ID-Protector在有效性、隐蔽性、鲁棒性方面的定量评估结果。

% % 为了评估我们的模型性能， 我们准备了两个测试集， 1是Celeb-A 的一个子集，没有参与训练。2.是从互联网上收集到的公众人物照片。 我们认为这些公众人物的照片在SD训练集里出现过，甚至出现在InstantID,IP-Adapter的训练集中， 是更难的攻击样本。

% \subsection{Experimental Setup}

% \textbf{Training data.} Our model utilizes the CelebA dataset. The dataset is the un-cropped CelebA dataset, which includes 200,000 images of people, encompassing close-ups, half-body, and full-body shots. This allows our model to generalize to various real-world scenarios.

% \textbf{Evaluation benchmarks}

% % 由于深度学习模型在训练过程中对数据集的特征进行了深入学习，模型在应对其训练数据集中的样本时通常更具鲁棒性。这使得在这些已知样本上进行对抗攻击的难度增加，尤其是在模型存在过拟合或采用了对抗训练的情况下。为了评估模型ID-Protector性能，我们使用以下3个benchmark:

% % 1. 我们从Celeb-A中划分出500张图像作为测试集，这部分图像没有参与ID-Protector encoder的训练。

% % 2. 我们从互联网收集200个公众人物照片作为公众人物测试集，这部分图像同样没有参与ID-Protector encoder的训练， 我们认为Stable diffusion, InstantID，CLIP 训练集包括这些样本， 因此攻击这些样本是较为困难的。

% % 3. 我们额外收集了一个素人测试集， 收集500张普通人的肖像（确保这些照片是新拍的）不会存在于SD, InstantID等方法的训练数据中。因此，这一设置能更准确的反映ID-Protector 真实使用场景的保护能力。

% Due to the deep learning model's extensive learning of the features within its training dataset, the model typically exhibits greater robustness when handling samples from this dataset. This increases the difficulty of conducting adversarial attacks on these known samples, particularly in cases where the model is overfitted or has undergone adversarial training.


% To evaluate our model, we employ several metrics and datasets:
% \begin{itemize}
%     \item \textbf{Celeb-A bench}: We selected 500 images from the Celeb-A dataset as our test set. These images were not used in the training of the ID-Protector encoder. 

%     \item \textbf{Public figures bench} : We collected 100 photos of public figures from the internet as a public figures test set. These images were also not used in the training of the ID-Protector encoder. We believe that Stable Diffusion and InstantID have encountered these IDs multiple times during training, making it the most challenging to attack these samples.
    
%     \item \textbf{Ordinary people bench} : Since Celeb-A is a publicly available dataset, we assume that the training sets of methods like Stable Diffusion, InstantID, and Arcface likely include these images, which would make the attack more difficult. Therefore, we additionally collected a "non-celebrity" test set, consisting of 500 portraits of ordinary people (ensuring that these photos were newly taken and not included in the training data of SD, InstantID, etc.). This setup more accurately reflects the protective capabilities of ID-Protector in real-world scenarios.
% \end{itemize}


% \textbf{Implementation details.} We trained our model on 200,000 portrait images using a learning rate decay strategy for 500 epochs. In the experiments, we selected InstantID, IP-Adapter, IP-Adapter plus, and PhotoMaker as the target models. All methods were tested with their recommended default settings to ensure fairness.

% \subsection{Evaluation benchmarks}
% % 本节介绍评价指标，我们采用以下指标衡量本文方法的有效性：
% \begin{itemize}
%     \item \textbf{Arcface Embedding Similarity}:  Arcface Embedding Similarity is a measure of how closely two facial images resemble each other by comparing their feature embeddings generated by the Arcface model, typically using cosine similarity to quantify the likeness between the two faces. 

%     \item \textbf{CLIP-I Score} : We collected 100 portraits of celebrities as a membership test set. These images were not used in the training of the ID-Protector encoder. However, Stable Diffusion recognizes these celebrities and is confident in generating their portraits given their names (e.g. Donald Trump). Through this, we demonstrate ID-Protector is powerful enough to even protect memberships of the generator training data.
    
% \end{itemize}

